Roadmap Document on Stochastic Analysis

This document was prepared as part of the MT-LAB research centre. The research centre studies the Modelling of Information Technology and is a VKR Centre of Excellence funded for five years by the VILLUM Foundation. You can read more about MT-LAB at its webpage www.MT-LAB.dk. The goal of the document is to serve as an introduction to new PhD students addressing the research goals of MT-LAB. As such it aims to provide an overview of a number of selected approaches to the modelling of stochastic systems. It should be readable not only by computers scientists with a background in formal methods but also by PhD students in stochastics that are interested in understanding the computer science approach to stochastic model checking. We have no intention of being encyclopedic in our treatment of the approaches or the literature. Rather we have made the selection of material based on the competences of the groups involved in or closely affiliated to MT-LAB, so as to ease the task of the PhD students in navigating an otherwise vast amount of literature. We have decided to publish the document in case other young researchers may find it helpful. The list of authors reflect those that have at times played a significant role in the production of the document.

==> preface.tex <==
%\newpage
\chapter*{Preface}\label{preface}
\addcontentsline{toc}{chapter}{Preface}
%\vspace{10 mm}
This document was prepared as part of the MT-LAB research centre. The
research centre studies the Modelling of Information Technology and is a
VKR Centre of Excellence funded for five years by the VILLUM Foundation.
You can read more about MT-LAB at its webpage www.MT-LAB.dk.

The goal of the document is to serve as an introduction to new PhD
students addressing the research goals of MT-LAB. As such it aims to
provide an overview of a number of selected approaches to the modelling of
stochastic systems. It should be readable not only by computers scientists
with a background in formal methods but also by PhD students in
stochastics that are interested in understanding the computer science
approach to stochastic model checking.

We have no intention of being encyclopedic in our treatment of the
approaches or the literature. Rather we have made the selection of
material based on the competences of the groups involved in or closely
affiliated to MT-LAB, so as to ease the task of the PhD students in
navigating an otherwise vast amount of literature.

We have decided to publish the document in case other young researchers
may find it helpful. The list of authors reflect those that have at times
played a significant role in the production of the document.

